When AUC Misleads: Polarization-Aware Evaluation of Deepfake Detectors under Domain Shift

Recent advances in generative AI, such as diffusion models and face-swapping tools, have enabled the creation of highly realistic deepfakes, leading to real-world harms including financial fraud and non-consensual explicit content. In response, deepfake detection has become an active research area, with recent methods increasingly focusing on improving generalization to unseen manipulations. This is typically evaluated using the Area Under the ROC Curve (AUC) measured separately across multiple datasets. However, such an evaluation fails to reflect real-world scenarios where detectors face a mixture of data sources and varying artifact types. To address this limitation, we introduce a novel metric, Cross-dataset AUC (Cross-AUC) that averages per-domain AUCs with a measure of prediction polarization for taking into account the robustness to domain shift. The polarization extent is quantified by the Wasserstein Distance between class score distributions. Cross-AUC not only assesses the generalization capabilities of deepfake detectors under domain shifts more realistically, but it is also interpretable as it better explains the reason behind a drop in performance. Experiments performed on seven benchmark datasets demonstrate its practical relevance.

==> secs/1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

Recent advances in generative AI, such as diffusion models and open-source face-swapping tools, have facilitated the creation of ultra-realistic forged facial images. Such manipulated data, also known as deepfakes, have already caused real harm, from financial scams~\cite{25m_video_call} to the diffusion of non-consensual explicit content~\cite{korea_deepfake_porn}.

In response to this threat, the field of deepfake detection has become a very active research topic~\cite{ff++,ict,ete_recons,sladd,sbi,fxray,aunet,laa_net,fakeformer,fakestormer,caddm,multi-attentional,forensicsadapter,fairnessDF}. Earlier methods mostly employ binary classifiers using standard deep learning architectures (\eg, Xception~\cite{xception}, EfficientNet~\cite{efn_net}) that learn to distinguish between real and fake data. However, these approaches tend to overfit specific artifact patterns introduced by the generation techniques used to create the fake training samples, resulting in limited generalization to unseen \textcolor{purple}{forgeries}. Solving this issue is crucial since new generative methods are constantly emerging, introducing distinct and inherently different artifact traces. To overcome this problem, recent state-of-the-art (SOTA) methods have adopted multi-task learning~\cite{cstency_learning,sladd,ete_recons,laa_net,caddm} and/or data synthesis strategies~\cite{sbi,sladd,fxray,ost,plug_play}, claiming increased robustness to unseen manipulations. To demonstrate the generalization capabilities of these methods, a cross-dataset evaluation protocol is typically followed, where different datasets are employed during training and testing phases~\cite{sbi,sladd,fxray,laa_net}. Given its robustness to imbalanced data, the Area Under the Receiver Operating Characteristic (ROC) Curve (AUC) is \textcolor{purple}{commonly adopted as the primary evaluation metric}~\cite{ict,ete_recons,sladd,sbi,fxray,aunet,laa_net,fakestormer,caddm,forensicsadapter}. \textcolor{purple}{It is computed separately on each test dataset and then averaged to provide an overall indicator of the detector's performance at deployment.}
Such an evaluation protocol, however, cannot fully reflect the relevance of a given deepfake detector in a real-world setting. \textcolor{purple}{Indeed, simply averaging independent scores implicitly assumes homogeneous and well-aligned score distributions across data sources, overlooking domain shifts and often overestimates and obscures actual generalization performance}. 

In practice, an effective detector should be able to handle uncontrolled deepfake data featuring \textcolor{purple}{anisotropic domain shifts from} different kinds of artifacts simultaneously, regardless of their original source. As such, it is likely that the encountered data resembles a mixture of multiple datasets. Therefore, evaluating AUC separately on each dataset, as commonly done, fails to capture this realistic condition. The AUC metric, which estimates the class separability of a binary classification model, can be high when evaluated on each dataset individually. However, it can drop drastically when considering two datasets incorporating a domain shift. \textcolor{purple}{As illustrated in Figure~\ref{fig:auc_weakness_vis}, mixing datasets A and B can cause a sharp AUC drop due to cross-domain score misalignment, whereas detectors with more consistent score separation remain stable on the combined set. This motivates an evaluation beyond per-dataset AUC that accounts for these distributional shifts.}



\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{figures/Cross-AUC.pdf}
\vspace{-1mm}
\caption{\textcolor{purple}{Example of dataset-dependent optimal thresholds for predictions on two datasets, A (top) and B (middle). Although both detectors achieve perfect $\text{AUC}=1$ when evaluated on each dataset separately, mixing A\&B (bottom) can cause a sharp AUC drop when scores are no longer consistently ordered across domains (Detector X), while a more stable detector preserves ordering and maintains $\text{AUC}=1$ (Detector Y). The anisotropic score distributions lead to incompatible optimal thresholds across datasets (\textcolor{OrangeRed}{red} range), highlighting cross-domain score misalignment and motivating polarization-aware evaluation.}}
\label{fig:auc_weakness_vis}
\vspace{-5mm}
\end{figure*}



Therefore, in this paper, we propose a new metric, called \textit{Cross-dataset AUC (Cross-AUC)}, that can better assess the generalization capabilities of deepfake detectors under domain shift. Cross-AUC relies on \textcolor{purple}{stability-aware aggregation of per-domain AUCs} across diverse datasets while taking into account the \textit{polarization} extent of the probability predictions. 
A stronger polarization of probability predictions (predictions closer to $0$ and $1$) suggests that the classes are more distinctly separated within the score space, and a fixed threshold is more likely to remain effective under varied conditions, contributing to enhanced generalization capabilities. 
The polarization extent is estimated using the Wasserstein Distance (WD) between the distributions of positive and negative probability predictions.
Consequently, the proposed Cross-AUC captures both the relative ranking performance (via the AUC) and the absolute separability of predictions (via the polarization), offering a more adequate estimation of generalization performance in real-world scenarios. 
We empirically show that the Cross-AUC is very close to the AUC measured on a combination of all the considered datasets, making it a practical measure for evaluating cross-dataset generalization.
\textcolor{purple}{Although testing on the Combined dataset reflects real-world settings as detectors will likely face mixed-domain inputs in practice, relying solely on the Combined AUC remains difficult to understand the reason behind the drop between average AUC and Combined AUC. Hence, Cross-AUC offers a better interpretation and understanding of the discrepancy between these two measures, demonstrating the important role of prediction polarization in the generalization capabilities of deepfake detectors. In other words, our work suggests that the separability extent between real and fake predictions across domains is crucial. This opens up a new direction for developing robust deepfake detectors that do not rely solely on the accuracy ranking as an evaluation criterion but consider also the prediction polarization across domains.}

% \textcolor{purple}{We empirically show that all considered detectors exhibit exaggerated expressiveness in performance estimated by the common averaged AUC as compared to the AUC measured on a combination of seven considered benchmarks. On the other hand, Cross-AUC closely tracks the value of the combined AUC. Notably, while such a combined AUC can play as a pseudo-realistic deployment-style assessment, it requires access to a mixed test set and characterizes a lack of explainability, \ie, it can not interpret which domains or which score mismatches drive the failure. In contrast, Cross-AUC can be computed from standard per-dataset evaluations only and by explicitly incorporating polarization, providing a diagnostic lens on generalization risk rather than a single opaque score.}
% \textcolor{purple}{Moreover, the metric is highly efficient for practical uses without the requirement of retraining or extra labels. Leveraging a lightweight cumulative density function, such as the Quantile, Cross-AUC can be suitable for both online and offline calculation with an incur of negligible computational runtime overhead.
% Although we scope the work only on deepfake detection, the metric's score-based formulation suggests that it may be potential to extend to other detection tasks under domain shift, a question we leave to future work.}

In summary, this work presents the following contributions:
\begin{itemize}
    % \item We discuss and analyze the sensitivity of AUC under domain shift and its unsuitability for \textcolor{purple}{fully} assessing the generalization capabilities of deepfake detectors.
    %  \item We introduce a new metric called \textit{Cross-dataset AUC (Cross-AUC)} to evaluate the generalization performance of deepfake detectors, taking into account the mean AUC across different datasets, as well as the polarization of probability predictions. 
    % \item We investigate the impact of prediction polarization between classes and show that similar AUC values can correspond to vastly different decision behaviors. This is quantified using the WD between score distributions.
    \item \textcolor{purple}{We analyze the behavior of AUC under domain shift and show that averaging per-dataset AUC scores can substantially overestimate the actual generalization of deepfake detectors on unconstrained mixed-domain data.}
    \item \textcolor{purple}{We introduce the Cross-AUC metric, a stability-aware aggregation of per-domain AUCs that is computed from standard per-dataset evaluations and uses prediction polarization to penalize cross-dataset score misalignment.}
    \item \textcolor{purple}{We investigate prediction polarization between classes and demonstrate that detectors with similar AUC can exhibit vastly different decision behaviors; we quantify this effect using a Wasserstein-distance-based measure and show how it is captured by Cross-AUC.}
    \item We conduct an experimental evaluation and analysis based on the proposed Cross-AUC for comparing deepfake detectors, including several recent SOTA methods~\cite{ff++,sladd,ete_recons,sbi,caddm,laa_net,forensicsadapter}, using seven well-known benchmarks~\cite{ff++,celeb_df,dfd,wdf,dfdcp,dfdc,DF40}.
\end{itemize}


==> tables/_overall_aucs.tex <==
\input{tables/_crossAUC_avgAUC_combinedAUC}


\noindent\textbf{Overall Performance Analysis.}
In Table~\ref {tabl:trimmed_results}, we evaluate seven deepfake detection models across seven datasets and a combined test set, using AUC, threshold stability (Top–\(\phi\)), and distributional separability quantified by the polarities using four different kinds of estimated densities.
It can be observed that ForensicAdapter~\cite{forensicsadapter} achieves the highest average AUC ($90.18\%$) and a high Combined AUC ($85.96\%$), indicating robust generalization across domains. It also consistently ranks among the best in distributional separability, reflecting reliable class boundaries.
LAA-Net~\cite{laa_net} attains the highest Combined AUC ($86.51\%$) and leads in terms of polarity across most datasets, suggesting strong discriminative capacity. However, its higher threshold variance suggests less stable decision boundaries in cross-domain settings.
RECCE~\cite{ete_recons} offers a strong balance between per-dataset AUC ($81.13\%$), Combined AUC ($76.91\%$), and low threshold variance, indicating consistent decision behavior across domains, though its class separability is slightly weaker.
SBI~\cite{sbi} and CADDM~\cite{caddm} perform moderately well in terms of both average and Combined AUC, but show less consistent threshold behavior and lower score separability.
Xception~\cite{xception} and SLADD~\cite{sladd} exhibit lower AUCs and weak generalization, confirming their limitations in complex, cross-domain settings. 
For a visual comparison of performance between detectors across datasets, see Figure~\ref{fig:radar_per_dataset}.
A more comprehensive view of performance with more evaluation metrics is reported in the supplementary materials.

%In summary, LAA-Net excels in overall detection accuracy, especially on mixed-domain inputs, while ForensicAdapter provides the most stable and generalizable performance across metrics.


\begin{figure}
    \centering
    \includegraphics[width=0.68\linewidth]{figures/dataset_auc_radar_all_splits.pdf}
    \vspace{-2mm}
    \caption{Methods results (AUC) for each dataset. Averaged AUC, AUC on the combined results, and the proposed Cross-AUC are also reported.}
    \label{fig:radar_per_dataset}
    \vspace{-4mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.68\linewidth]{figures/model_auc_radars.pdf}
    \vspace{-2mm}
    \caption{Direct comparison of average AUC, combined AUC, and the proposed Cross-AUC on the studied methods.}
    \label{fig:radar_per_method}
    \vspace{-3mm}
\end{figure}



\input{tables/different_mean_table}


\vspace{1mm}
\noindent\textbf{Polarization Robustness under Domain Shift.} 
We compare the polarization scores of each model by looking at their average values across individual datasets and their value on the combined dataset, as shown in Table~\ref{tabl:trimmed_results}. In general, most models show a lower polarization score on the combined set compared to the average across separate datasets.
LAA-Net has the highest average polarization (e.g., average $W_Q$: $0.486$) and performs well on several datasets such as CDF, DFW, DFDCP. However, it also shows the largest drop in the combined setting, with its score decreasing to $0.318$. 
ForensicsAdapter has a slightly lower average $0.402$, but its combined score remains relatively high $0.336$, showing less difference between the two. This suggests that its behavior is more consistent across domains.
RECCE shows moderate scores in both settings ($0.273$ average, $0.232$ combined) with only a small change. SBI, CADDM, and Xception achieve strong scores on specific datasets (e.g., FF++, DFD), but their combined scores are notably lower. SLADD has low scores in both average $0.032$ and combined $0.014$ cases, with very little variation. These observations are further supported by Figure~\ref{fig:full_pred_patterns}.

Overall, most models show a drop in polarization when moving from individual datasets to the combined set. This gap provides a simple indication of how much a model's ability to separate real and fake predictions is affected by domain shift. These results suggest that evaluating the polarization on mixed-domain inputs is useful to understand the robustness of the model. 

% We compare the global polarity of each model by comparing their averaged polarities (calculated on individual datasets) and the one on the combined multi-domain set in Table~\ref{tabl:trimmed_results}.
% The drop from global polarity to combined polarity reveals that per-dataset polarization may overstate a model’s true capability, while combined polarity offers a more realistic reflection of generalization in real-world, mixed-domain settings.
% LAA-Net achieves the highest global polarity (e.g., average $W_\text{Q}$: $0.486$), reflecting strong separability under controlled conditions. It performs especially well on CDF2, DFW, and DFDCP, but exhibits the largest drop in the combined setting ($W_\text{Q}$: $0.318$), indicating that its confidence margin drops under domain shift.
% ForensicAdapter ranks slightly lower in global polarity (e.g., $0.402$) but shows the strongest polarity on the combined set ($W_\text{Q}$: $0.336$), with minimal degradation.
% This stability reflects domain-invariant polarization and supports its superior generalization.
% RECCE maintains moderate polarity values with minimal drop ($W_\text{Q}$: $0.273$ $\rightarrow$ $0.232$), indicating consistent, although less pronounced, score separation.
% It performs reliably on DFD and DF40, albeit with tighter margins.
% SBI, CADDM, and Xception register strong polarity on certain datasets (e.g., DFD, FF++), but suffer from substantial declines in the combined setting, suggesting overfitting.
% SLADD maintains low polarity across all conditions ($W_{Q}$: $0.032$ $\rightarrow$ $0.014$), indicating limited ability to distinguish real from fake across domains.
% These observations are further supported by Figure~\ref{fig:full_pred_patterns}.



% In summary, the gap between global polarity and the polarity on the combined dataset offers a useful indication on how well score separability is maintained under domain shift.
% These observations support the relevance of evaluating polarities under mixed-domain conditions for assessing robustness.

\vspace{1mm}
\noindent\textbf{Conventional Average AUC is Overoptimistic.}
Table~\ref{table:AUC_results} compares the conventional average AUC across individual datasets (\(\text{AUC}_a\)) with the AUC measured on the combined test set (\(\text{AUC}_c\)).
Across all models, \(\text{AUC}_a\) is consistently higher than \(\text{AUC}_c\), with gaps ranging from $1.77 \%$ (LAA-Net) to over $12 \%$ (SLADD).
This consistent drop highlights that average AUC often overstates generalization, as it reflects performance under domain-specific conditions with implicit per-domain advantages.
However, models in deployment encounter inputs from mixed or unknown distributions, more closely represented by the combined test set.
The lower \(\text{AUC}_c\) values expose how model predictions degrade under such conditions, revealing weaknesses that per-domain averages mask.
To address this, we include our proposed Cross-AUC.
In all cases, Cross-AUC is significantly closer to \(\text{AUC}_c\) than \(\text{AUC}_a\), often reducing the error by more than $80\%$.
This demonstrates the effectiveness of the proposed metric in approximating real-world performance.
These results confirm that relying solely on average AUC can be misleading. Evaluating on combined distributions or computing such a metric is essential for assessing generalization capabilities.

\input{tables/_polarization_estimator}

\input{tables/_ood}

\input{tables/_different_lambda}


\vspace{1mm}
\noindent\textbf{AUC Generalizability with Cross-AUC}. 
To assess how well performance on individual datasets generalizes to realistic, multi-domain deployment, we analyze the gap between predicted Cross-AUC and the combined AUC (\(\text{AUC}_c\)), as shown in Table~\ref{table:AUC_results}.
Unlike the conventional average AUC (\(\text{AUC}_a\)), which consistently overestimates performance under distribution shift, Cross-AUC is explicitly designed to estimate generalization using only per-dataset AUCs and score-level polarization, measured from Table~\ref{tabl:trimmed_results}.
Across all models, Cross-AUC consistently aligns more closely with \(\text{AUC}_c\) than \(\text{AUC}_a\), achieving the smallest difference (\(\Delta_\text{Cross-AUC}\)) in all cases. 
An alternative radar-based view of the comparison is given in Figure~\ref{fig:radar_per_method}.
Occasional \textit{rank reversals} are also observed (e.g., ForensicsAdapter vs. LAA-Net; see Supplementary), where a model with the highest average AUC underperforms on both Combined AUC and Cross-AUC.
Overall, these results demonstrate that Cross-AUC, computed based on per-domain performance and polarization, offers a robust and practical estimator of cross-domain generalization.


\vspace{1mm}
\noindent\textbf{Cross-AUC versus H-score.} H-score~\cite{h-score} was originally designed for universal domain adaptation as the harmonic mean of accuracies on common and unknown classes. To align with our setting, we replace accuracy with per-dataset AUC. While this adaptation provides a useful baseline, H-score does not reflect the effect of domain-dependent threshold shifts. Consequently, its estimates remain farther from the combined AUC compared to Cross-AUC (Table~\ref{table:AUC_results}).


\vspace{1mm}
\noindent\textbf{Out-of-Distribution (OOD) Evaluation with MagicBrush.}
We further evaluate generalization with MagicBrush~\cite{magicbrush}, which contains manipulation types unseen in prior benchmarks. In addition to testing detectors on MagicBrush alone, we also include it as an eighth dataset and recompute all metrics across the expanded pool. Table~\ref{tab:ood} shows that the gap between average AUC and the combined AUC becomes even more pronounced, while Cross-AUC remains consistently close to the combined AUC. This demonstrates that Cross-AUC provides a reliable estimate not only under controlled benchmarks but also when truly novel manipulations are integrated into evaluation.



\subsection{Ablation Studies}

\noindent\textbf{Effect of Mean Function in Cross-AUC Estimation.}
Table~\ref{tab:mean_aucs} presents an ablation study comparing three averaging functions ($\Psi$), harmonic, arithmetic, and geometric, used in our Cross-AUC.
We evaluate their effectiveness by measuring the absolute difference with combined AUC (\(\text{AUC}_c\)).
The results show that the harmonic mean consistently produces closest results, achieving the lowest difference (\(\Delta\)) in $6$ out of $7$ models. For example, it predicts within $0.42$ points for Xception, $1.19$ for SLADD, and only $0.04$ for LAA-Net. %Even for models with high variability across domains (e.g., CADDM), the harmonic mean outperforms both the arithmetic and geometric alternatives.
%These findings suggest that the harmonic mean more effectively balances domain-specific performance, down-weighting overly confident scores in unstable domains. In contrast, the arithmetic mean tends to inflate the estimate, particularly in models with uneven domain behavior. The geometric mean performs moderately but does not consistently match the combined AUC.

%Overall, this analysis supports the use of the harmonic mean as the default aggregation strategy in Cross-AUC, offering a robust and conservative approximation of generalization performance.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/tsne_combined_all.pdf}
%     \caption{The t-SNE~\cite{tsne} visualization for each detector. These detectors are trained on FF++~\cite{ff++}.}
%     \vspace{-5mm}
%     \label{fig:tsne}
% \end{figure}



% \textbf{Feature Space.} We use t-SNE~\cite{tsne} to visualize the latent features extracted from the final layer of each detector on the combined test set. As shown in Figure~\ref{fig:tsne}, none of the models produce clearly separated feature clusters when exposed to mixed or unseen domains. This illustrates the difficulty of the proposed evaluation setting and underscores the need for more rigorous, distribution-aware assessment protocols in realistic deployment scenarios.


\vspace{1mm}
\noindent\textbf{Cross-AUC with Different Polarization Estimators.} 
We further examine the effect of replacing the Wasserstein Distance in Cross-AUC with alternative separability measures. As shown in Table~\ref{table:different_estimators}, both Wasserstein and KL-based Cross-AUC remain closely aligned with the combined AUC, whereas the Jensen-Shannon (JS) variant yields less consistent estimates. This suggests that while Cross-AUC is generally robust to the choice of estimator, Wasserstein offers the most stable approximation under distribution shift.



\vspace{1mm}
\noindent\textbf{Effect of Balancing Factor $\lambda$.}
We also examine the influence of the balancing factor $\lambda$ in Cross-AUC, which controls the trade-off between mean AUC and polarization. As shown in Table~\ref{tab:different_lambda}, very small $\lambda$ values reduce Cross-AUC to a simple average AUC and thus deviate from the combined AUC, while excessively large $\lambda$ values overweight polarization and also degrade alignment. A mid-range choice ($\lambda$ $\approx$ $0.5$) consistently yields the closest approximation to AUC$_c$, confirming that Cross-AUC is robust provided $\lambda$ is set within a reasonable range.




\vspace{1mm}
\noindent\textbf{Runtime Analysis.}
We report runtime for different polarization estimators in Table~\ref{tab:runtime}. Non-parametric variants ($W_{\text{KDE}}$, $W_\text{Q}$) incur only millisecond-level overhead, while the GMM-based estimator ($W_{\text{GMM}}$) is slower by orders of magnitude. Nevertheless, all variants remain practical for offline evaluation, and the default Wasserstein implementation achieves a very good balance between efficiency and fidelity.

\input{tables/_runtime}



\subsection{Potential Impact on the Research Community}
This work introduces a simple yet effective framework for assessing model generalization under domain shift. By moving beyond conventional per-domain metrics and incorporating score-level polarization, Cross-AUC can be used as a replacement for average AUC, which can obscure real-world failure cases. As such, it provides researchers with a more reliable estimate of performance under uncontrolled conditions.  More broadly, this highlights the need for a shift in the community toward evaluation protocols that prioritize reliability and robustness across domains over isolated benchmarks.

